Covert channel detection using Information Theory

This paper presents an information theory based detection framework for covert channels. We first show that the usual notion of interference does not characterize the notion of deliberate information flow of covert channels. We then show that even an enhanced notion of "iterated multivalued interference" can not capture flows with capacity lower than one bit of information per channel use. We then characterize and compute the capacity of covert channels that use control flows for a class of systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{K. Chatzikokolakis and V. Cortier (Ed.): 8th International Workshop\\
on Security Issues in Concurrency (SecCo 2010)\\
EPTCS 51, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.51.3}{10.4204/EPTCS.51.3}}

